Quantitative group testing with a fixed shore: sharp asymptotics and exact formulas

Two disjoint sets each contain one defective item. A test reports how many defectives lie in a chosen subset, and its choice may depend on earlier answers. We determine the largest searchable second set for every test budget when the first set has six, seven or eight items, extending the known answers through five. For six items, every optimal first test splits them four and two once at least nine tests are available. For eight, the exact formula gains one item over a quadratic correction every three tests. We explain the rounding in an optimal strategy and prove a matching bound over all strategies using exact rational certificates. For an arbitrary fixed first set, we determine the degree and leading coefficient of the loss from the binary bound.

==> atlas-colors.tex <==
\usetikzlibrary{patterns}
\definecolor{branchtwozero}{HTML}{5098E8}
\definecolor{branchthreetwo}{HTML}{F0A020}
\definecolor{branchthreezero}{HTML}{F86870}
\definecolor{branchfourtwo}{HTML}{B0E028}
\definecolor{branchfourzero}{HTML}{C070D0}
\definecolor{earlyforest}{HTML}{28B858}
\definecolor{branchfivezero}{HTML}{A08868}
\definecolor{answerzero}{HTML}{F8E0A8}
\definecolor{answerone}{HTML}{90C8C7}
\definecolor{answertwo}{HTML}{F8A8E0}
